Simplifying Data Integration: SLM-Driven Systems for Unified Semantic Queries Across Heterogeneous Databases

The integration of heterogeneous databases into a unified querying framework remains a critical challenge, particularly in resource-constrained environments. This paper presents a novel Small Language Model(SLM)-driven system that synergizes advancements in lightweight Retrieval-Augmented Generation (RAG) and semantic-aware data structuring to enable efficient, accurate, and scalable query resolution across diverse data formats. By integrating MiniRAG's semantic-aware heterogeneous graph indexing and topology-enhanced retrieval with SLM-powered structured data extraction, our system addresses the limitations of traditional methods in handling Multi-Entity Question Answering (Multi-Entity QA) and complex semantic queries. Experimental results demonstrate superior performance in accuracy and efficiency, while the introduction of semantic entropy as an unsupervised evaluation metric provides robust insights into model uncertainty. This work pioneers a cost-effective, domain-agnostic solution for next-generation database systems.

==> sections/draft.tex <==
The integration of heterogeneous databases into a unified querying framework remains a critical challenge, particularly in resource-constrained environments. This paper presents a novel Small Language Model (SLM)-driven system that synergizes advancements in lightweight Retrieval-Augmented Generation (RAG) and semantic-aware data structuring to enable efficient, accurate, and scalable query resolution across diverse data formats. By integrating MiniRAG’s semantic-aware heterogeneous graph indexing and topology-enhanced retrieval with SLM-powered structured data extraction, our system addresses the limitations of traditional methods in handling Multi-Entity Question Answering (Multi-Entity QA) and complex semantic queries. Experimental results demonstrate superior performance in accuracy and efficiency, while the introduction of semantic entropy as an unsupervised evaluation metric provides robust insights into model uncertainty. This work pioneers a cost-effective, domain-agnostic solution for next-generation database systems.

==> sections/refs.tex <==
\begin{thebibliography}{00}

\bibitem{gao2023survey} Y. Gao, Y. Xiong, X. Gao, K. Jia, J. Pan, Y. Bi, Y. Dai, J. Sun, and H. Wang, ``Retrieval-augmented generation for large language models: A survey,'' arXiv preprint arXiv:2312.10997, 2023.
\bibitem{liu2024Mobilellm} Z. Liu, C. Zhao, F. Iandola, C. Lai, Y. Tian, I. Fedorov, Y. Xiong, E. Chang, et al., ``Mobilellm: Optimizing sub - billion parameter language models for on-device use cases,'' in Proceedings of the International Conference on Machine Learning (ICML), 2024.
\bibitem{Arora2024EVAPORATE} S. Arora, B. Yang, S. Eyuboglu, A. Narayan, A. Hojel, I. Trummer, and C. Re, ``Language Models Enable Simple Systems for Generating Structured Views of Heterogeneous Data Lakes,'' Proceedings of the VLDB Endowment, vol. 17, no. 2, pp. 92-105, 2023.
\bibitem{fan2025minirag} T. Fan, J. Wang, X. Ren, and C. Huang, ``MiniRAG: Towards Extremely Simple Retrieval-Augmented Generation,'' arXiv:2501.06713 [cs.AI], Jan. 2025, https://arxiv.org/abs/2501.06713.
\bibitem{Kuhn2023Semantic} L. Kuhn, Y. Gal, and S. Farquhar, ``Semantic Uncertainty: Linguistic Invariances for Uncertainty Estimation in Natural Language Generation,'' arXiv:2302.09664 [cs.CL], Feb. 2023, [Online]. Available: https://arxiv.org/abs/2302.09664.
\bibitem{Patel2024LOTUS} L. Patel, S. Jha, C. Guestrin, and M. Zaharia, ``LOTUS: Enabling Semantic Queries with LLMs over Tables of Unstructured and Structured Data,'' arXiv:2407.11418, 2024.
\bibitem{Farquhar2024Detecting} S. Farquhar, J. Kossen, L. Kuhn, and Y. Gal, ``Detecting Hallucinations in Large Language Models Using Semantic Entropy,'' NATURE, vol. 630, pp. 2024.
\bibitem{edge2024local} D. Edge, H. Trinh, N. Cheng, J. Bradley, A. Chao, A. Mody, S. Truitt, and J. Larson, ``From Local to Global: A Graph RAG Approach to Query-Focused Summarization,'' CoRR, vol. abs/2404.16130, 2024.
\bibitem{Tang2024graphgpt} J. Tang, Y. Yang, W. Wei, et al., ``GraphGPT: Graph Instruction Tuning for Large Language Models,'' arXiv:2310.13023 [cs.CL], 2023, [Online]. Available: https://doi.org/10.48550/arXiv.2310.13023.
\bibitem{he2024gretriever} X. He, Y. Tian, Y. Sun, N. V. Chawla, T. Laurent, Y. LeCun, X. Bresson, and B. Hooi, ``G-Retriever: Retrieval-Augmented Generation for Textual Graph Understanding and Question Answering,'' arXiv:2402.07630 [cs.LG], 2024, [Online]. Available: https://arxiv.org/abs/2402.07630
\bibitem{guan2023mitigating} X. Guan, Y. Liu, H. Lin, Y. Lu, B. He, X. Han, and L. Sun, ``Mitigating Large Language Model Hallucinations via Autonomous Knowledge Graph - based Retrofitting,'' arXiv:2311.13314 [cs.CL], 2023, [Online]. Available: https://arxiv.org/abs/2311.13314
\bibitem{Chan2024RQRAGLT} C.-M. Chan, C. Xu, R. Yuan, H. Luo, W.Xue, Y. -T. Guo, and J. Fu, ``RQ-RAG: Learning to Refine Queries for Retrieval Augmented Generation,'' arXiv:2404.00610, 2024, [Online]. Available:https://api.semanticscholar.org/CorpusID:268819582.

\end{thebibliography}
